MT-PCR: Hybrid Mamba-Transformer Network with Spatial Serialization for Point Cloud Registration

Point cloud registration (PCR) is a fundamental task in 3D computer vision and robotics. Most learning-based PCR methods rely on Transformer architectures, which suffer from quadratic computational complexity. This limitation restricts the resolution of point clouds that can be processed, inevitably leading to information loss. In contrast, Mamba, a recently proposed model based on state-space models, achieves linear computational complexity while maintaining strong long-range contextual modeling capabilities. However, directly applying Mamba to PCR tasks yields suboptimal performance due to the unordered and irregular nature of point cloud data. To address these challenges, we propose MT-PCR, the first point cloud registration framework that integrates Mamba and Transformer modules. Specifically, we serialize point cloud features using Z-order space-filling curves to enforce spatial locality, enabling Mamba to better model the geometric structure of the inputs. Additionally, we remove the order-indicator module commonly used in Mamba-based sequence modeling, leading to improved performance in our setting. The serialized features are then processed by an optimized Mamba encoder, followed by a Transformer-based feature refinement stage. Extensive experiments on multiple benchmarks demonstrate that MT-PCR outperforms Transformer-based and other state-of-the-art methods in both accuracy and efficiency, significantly reducing GPU memory usage and FLOPs.

==> sec/06_acknowledgments.tex <==
% DO NOT INCLUDE ACKNOWLEDGMENTS IN AN ANONYMOUS SUBMISSION TO SIGGRAPH
\begin{acks}

\end{acks}










==> sec/07_biography.tex <==
% \section{Biography Section}
% If you have an EPS/PDF photo (graphicx package needed), extra braces are
%  needed around the contents of the optional argument to biography to prevent
%  the LaTeX parser from getting confused when it sees the complicated
%  $\backslash${\tt{includegraphics}} command within an optional argument. (You can create
%  your own custom macro containing the $\backslash${\tt{includegraphics}} command to make things
%  simpler here.)
 
% \vspace{11pt}

% \bf{If you include a photo:}\vspace{-33pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/BingxiLiu.png}}]{Bingxi Liu}
received the B.S. degree from the China
University of Mining and Technology in 2019, and the M.S. degree from the University of Chinese Academy of Sciences (UCAS) in 2022. He is currently pursuing the Ph.D. degree under the supervision of Prof. Hong Zhang at Southern University of Science and Technology (SUSTech). His research interests include visual place recognition and localization.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/AnLiu.jpg}}]{An Liu}
	is currently pursuing the B.S. degree in Computer Science and Technology (Excellence Program) at Chongqing University, with an expected graduation in 2026. His research interests include 3D vision, point cloud registration, and multi-modal perception for autonomous driving.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/HaoChen.jpg}}]{Clavin Chen}
	is currently a Ph.D. student at the University of Cambridge, supervised by Prof. Chao Li. He is also an active researcher at the MI+x Lab, University of Birmingham, working with Prof. Jianbo Jiao. He is from the Cantonese region in southeastern China. His research focuses on multi-modal representation learning and reducing supervision dependence, with applications in computer vision and healthcare, particularly in image processing, segmentation and generation.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/HuaqiTao.jpg}}]{Huaqi Tao}
	is currently pursuing the M.Sc. degree in the Robotics and Computer Vision Lab under the supervision of Prof. Hong Zhang at Southern University of Science and Technology (SUSTech). He received the B.Eng. degree from Guangxi University in 2024. His research interests include robotics and computer vision.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/JinqiangCui.png}}]{Jinqiang Cui}
received the B.E. and M.Sc. degrees in mechatronic engineering from Northwestern Polytechnical University, Xi'an, China, in 2005 and 2008, respectively, and the Ph.D. degree in electrical and computer engineering from the National University of Singapore, Singapore, in 2015. He was a Sensor Design Engineer with HSG-IMIT, Freiburg im Breisgau, Germany, from 2008 to 2010. He was the Chief Technology Officer for an unmanned aerial vehicle startup company from 2016 to 2019. He is currently with the Peng Cheng Laboratory, Shenzhen, China. His research interests include simultaneous localization and mapping, 3-D reconstruction, and intelligent multi-robot systems. Dr. Cui is an associate editor for Unmanned Systems.

\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/YiQunWang.jpg}}]{Yi-Qun Wang}
	is currently an Associate Professor at the College of Computer Science, Chongqing University. He received the B.S. degree from Chongqing University in 2016, and the Ph.D. degree from the National Laboratory of Pattern Recognition (NLPR), Institute of Automation, Chinese Academy of Sciences (CASIA), and the University of Chinese Academy of Sciences (UCAS). He was a Postdoctoral Research Fellow with the Visual Computing Center (VCC) at King Abdullah University of Science and Technology (KAUST), working with Professor Peter Wonka. His research interests include visual computing and pattern recognition.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/HongZhang2.png}}]{Hong Zhang}
	is a Chair Professor in the Department of Electronic and Electrical Engineering at Southern University of Science and Technology (SUSTech). Prior to joining SUSTech, he was a Professor in the Department of Computing Science at the University of Alberta for over 30 years. He received the B.Sc. degree from Northeastern University (USA) and the Ph.D. degree from Purdue University, followed by an 18-month postdoctoral training at the University of Pennsylvania. He is active in the international robotics community (ICRA \& IROS) and has been elected Fellow of IEEE and Fellow of the Canadian Academy of Engineering.	His research interests include robotics, computer vision, and image processing, with a focus on visual robot navigation.
\end{IEEEbiography}




==> sec/XX_response.tex <==


\noindent
Dear Chairs, Editors, and Reviewers:

\vspace{0.2cm}
\noindent

We are pleased to submit a revised version of our manuscript, “MT-PCR: Hybrid Mamba-Transformer Network with Spatial Serialization for Point Cloud Registration,” which was accepted at CVM 2026 and recommended for submission to IEEE Transactions on Visualization and Computer Graphics (TVCG).

We sincerely thank the reviewers for their constructive comments and suggestions. Following the CVM 2026 reviews, we have carefully revised the manuscript to address all concerns and to further strengthen the work to meet TVCG’s high publication standards.

Below, we summarize how we have responded to each reviewer’s comments:

\textbf{Response to Reviewer WIxkxO8r (R1)}

Comment 1 \& 2:
We provided additional clarifications and elaborations to address these questions.

Comment 3:
We revised the wording in the corresponding part of the manuscript to remove ambiguity.

Comment 4:
We added new experiments to strengthen the empirical evidence.

\textbf{Response to Reviewer 8OmNUZ8r (R2)}

Comment 1 \& 3:
We added further explanations and clarifications to directly answer these questions.

Comment 2:
We conducted additional experiments and incorporated the results into the revised manuscript.

\textbf{Response to Reviewer Wwtm9Iqc (R3)}

Comment 1 \& 2:
We provided clarifications and expanded the discussion to address these questions.

Comment 3:
We performed additional experiments and included an extended discussion.

In addition to the above, we carefully proofread the manuscript and improved the organization and writing for clarity. We believe the revised paper is substantially strengthened and is now better positioned to meet the rigorous expectations of TVCG.

Thank you for considering our revised submission. We appreciate your time and effort, and we look forward to the review process.

\vspace{0.2cm}
\noindent
Yours sincerely,


\noindent
Bingxi Liu, Hong Zhang

\noindent
SUSTech, Shenzhen, China



% \section*{Response to the Editor} 
% \begin{cmt*}{}{}
% Editor comments.
% \end{cmt*}

% \vspace{0.1cm}
% \noindent
% \underline{\textbf{Response:}}
% \vspace{0.2cm}

% Our response.

% Reviewer

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Reviewer 1
% \newpage
\section*{Response to Reviewers} 

%%%%%%%%%%%%% Comment
\begin{cmt*}{R1C1}{}
While Table 7 shows performance drops when the order indicator is added, the explanation that it ``artificially breaks spatial adjacency'' is speculative. In works like PointMamba, the order indicator resolves ambiguity when multiple traversal orders are used. Since MT-PCR uses only one Z-order sequence, the indicator may indeed be redundant. However, this should be explicitly clarified. A more rigorous analysis, for example visualizing attention or hidden states with and without the indicator, would strengthen the claim.
\end{cmt*}

\begin{cmt*}{R2C1}{}

The authors mention removing the ``Order Indicator'' token, which is a significant deviation from previous works like PointMamba, but they bury the justification for this only in the ablation study (Section 5.6). Since this is a core architectural decision to support the unidirectional scan, it really needs to be front and center in the Method section so the readers won't be confused about the flow.

\end{cmt*}

\vspace{0.1cm}
\noindent
\underline{\textbf{Response:}}
\vspace{0.2cm}

In prior work such as PointMamba, the Order-Indicator module was necessary because the model used two spatial curves (e.g., Hilbert and T-Hilbert) within the same Mamba encoder to perform bidirectional modeling. Without explicit order distinction, the mixed sequences would interfere with each other in the latent space, degrading performance. In contrast, our method performs all bidirectional information exchange in a subsequent cross-attention module, while the Mamba encoder operates only on a unidirectional sequence generated through dynamic serialization. This design preserves the geometric continuity of the point cloud from the beginning. Introducing an Order-Indicator in our case would artificially break spatial adjacency, weakening Mamba’s ability to capture local topology. As shown in Table 6, adding the Order-Indicator leads to a 0.8\% drop in RR, confirming its negative impact. Therefore, we chose to remove this module to maximize the preservation of geometric structure during Mamba processing.

\vspace{0.3cm}


\begin{cmt*}{R1C2}{}

Lack of comparison with concurrent Mamba-based 3D methods: The paper cites PointMamba and Mamba3D but does not include them in the main comparison (Table 1). Given that these are the closest architectural relatives, their omission raises fairness concerns. The authors should either reproduce their results on 3DMatch or explain why they are not comparable (e.g., different task formulation).

\end{cmt*}
\vspace{0.1cm}
\noindent
\underline{\textbf{Response:}}
\vspace{0.2cm}

We clarified that PointMamba and Mamba3D were excluded from the main comparison because they are specialized for point cloud analysis tasks (e.g., classification, segmentation), which fundamentally differ from point cloud registration. While these methods excel at extracting semantic features for object recognition, they lack the essential mechanisms required for registration, such as dense correspondence matching, overlap detection, and transformation regression. Adapting them for our task would necessitate significant architectural redesign (e.g., replacing classification heads with matching modules) and retraining, effectively treating them as generic backbones rather than comparable registration baselines. Therefore, we focused our evaluation on state-of-the-art methods specifically tailored for the registration task to ensure a fair and relevant benchmark. 

\vspace{0.3cm}


\begin{cmt*}{R1C3}{}

Ambiguity in “hybrid” Mamba–Transformer integration: Figure 3 suggests Mamba is used only at the superpoint level (coarse stage), while Transformer handles fine matching. However, the text states “stacked Mamba blocks” and “Transformer-based refinement” without clarifying whether features from both branches are fused or processed sequentially. A clearer architectural diagram or pseudocode would improve reproducibility.

\end{cmt*}
\vspace{0.1cm}
\noindent
\underline{\textbf{Response:}}
\vspace{0.2cm}

We apologize for the lack of clarity in the text. We clarify that the Mamba and Transformer components are not separate parallel branches but are integrated into a fused processing architecture. Specifically, the features from the two inputs are processed sequentially through the Mamba block (for global context) and the Transformer block (for refinement). This sequential integration effectively fuses the strengths of both. \textbf{We have updated in the revision to explicitly illustrate this sequential yet fused design.}

\vspace{0.3cm}


%%%%%%%%%%%%% Comment 1.3
\begin{cmt*}{R1C4}{}

Computational advantage may be overstated: The FLOPs comparison (Figure 2, Table 3) is measured against dense Transformer baselines (e.g., GeoTransformer). However, many recent PCR methods (e.g., Predator, CoFiNet) use sparse correspondences or local attention, which already mitigate quadratic complexity. The paper should compare against efficient Transformers (e.g., with local windowing or token pruning) to isolate the benefit of Mamba itself.

\end{cmt*}
\vspace{0.1cm}
\noindent
\underline{\textbf{Response:}}
\vspace{0.2cm}

We appreciate the suggestion to expand the efficiency baselines. \textbf{In our revision, we extended the analysis by adding CoFiNet (a representative sparse method) for comparison.} The results (see Table below) confirm that our computational advantage is substantial: at 1024 tokens, CoFiNet requires 3.7x more GFLOPs than MT-PCR and encounters Out-of-Memory (OOM) errors at 1536 tokens, proving that sparse strategies alone do not fully resolve the bottleneck. Regarding the suggestion to include Predator in this specific scalability study, we respectfully excluded it because it relies on a Graph Neural Network (GNN) backbone. Our efficiency analysis aims to isolate the architectural trade-off between Mamba's linear complexity and Attention's quadratic complexity in sequence modeling. Including GNNs would introduce confounding factors (e.g., dynamic graph construction) with fundamentally different scaling laws, obscuring the direct comparison. However, please note that Predator remains fully included in our main accuracy benchmarks (Tables 1 and 2).

\vspace{0.3cm}

\begin{cmt*}{R2C2}{} 

Second, I’d like more clarity on rotation invariance. We know Z-order curves change drastically if you rotate the input, yet your model handles rotation very well (0.16 degree error in table 2). I suspect the heavy lifting job is actually being done by the KPConv backbone and the permutation-invariant Cross-Attention module, masking the instability of the Z-order sequence, but it would be great if the authors could explicitly analyze this trade-off in the text.

\end{cmt*}
\vspace{0.1cm}
\noindent
\underline{\textbf{Response:}}
\vspace{0.2cm}

We acknowledge that Z-order sequences are coordinate-dependent;\textbf{ however, our new ablation experiments (see Table 1) demonstrate that the Mamba module actively enhances, rather than hinders, rotation estimation.} Specifically, removing the Mamba encoder causes the Relative Rotation Error (RRE) to deteriorate significantly from 0.161° to 0.273°, refuting the hypothesis that the KPConv backbone and cross-attention merely "masks" instability. Furthermore, removing the Z-order strategy (w/o zorder) increases RRE to 0.174°, indicating that despite sequence variations under rotation, the spatial locality preserved by Z-order provides a superior inductive bias for global geometric modeling compared to unstructured inputs. This confirms that the Mamba encoder is indispensable for high-precision rotational alignment, capturing global context that local descriptors alone cannot resolve.

\begin{table}[t]
\small
\centering
\caption{\textbf{Ablation Study on Rotation Estimation Components.}}
\label{tab:zorder}
\begin{adjustbox}{}
\begin{tabular}{l|ccc}
\toprule
Setting  & RR (\%) & RRE ($^\circ$) & PTE (cm)  \\
\midrule
w/o zorder & \textbf{100.0} & 0.174 & 2.64 \\
w/o mamba & \textbf{100.0} & 0.273 & 2.56 \\
MT-PCR & \textbf{100.0} & \textbf{0.161} & \textbf{2.55} \\
\bottomrule
\end{tabular}
\end{adjustbox}

\end{table}


\vspace{0.3cm}

\begin{cmt*}{R2C3}{} 

Finally, while using Z-order curves is effective, please be careful not to oversell the novelty of the curve itself, as it is a standard tool (and it has been used in Transformers very often, mostly for efficiency purposes); the novelty really lies in why it is necessary for the inductive bias of Mamba.

\end{cmt*}
\vspace{0.1cm}
\noindent
\underline{\textbf{Response:}}
\vspace{0.2cm}

We fully agree that the Z-order curve is a standard tool. \textbf{In our revision, we have toned down claims about the curve itself and instead emphasized our specific insigh}t: Z-order provides the necessary inductive bias for Mamba. Unlike Transformers where it primarily optimizes efficiency, for Mamba, the spatial-to-temporal continuity enforced by Z-order is a prerequisite for effective geometric modeling on unstructured data.


\vspace{0.3cm}


\begin{cmt*}{R3C1}{} 

The results in Table 1 for the 3DMatch and 3DLoMatch datasets only consider Registration Recall, but not the RTE and RRE metrics that were also considered in other papers. (Interestingly, Table 2 includes all three metrics for another dataset; why not show the same for Table 1?). Without these additional metrics, we cannot get a full picture of the accuracy on 3DMatch and 3DLoMatch.

\end{cmt*}
\vspace{0.1cm}
\noindent
\underline{\textbf{Response:}}
\vspace{0.2cm}

We strictly followed the standard evaluation protocol established by previous state-of-the-art methods (e.g., Predator, GeoTransformer, CoFiNet) on the 3DMatch/3DLoMatch benchmarks, which primarily report Registration Recall (RR).
Unlike the odometry-focused KITTI benchmark (where trajectory drift is key), 3DMatch is a loop-closure benchmark where success is binary (pass/fail based on a threshold). Reporting average RTE/RRE on this dataset can be misleading, as it is typically calculated only on "successful" pairs; methods can artificially lower average error by failing on difficult cases. Therefore, RR is widely accepted as the most robust and fair metric for this specific benchmark. We ensured our Table 1 aligns exactly with the metrics reported by the baselines to ensure a fair, apples-to-apples comparison.

% \vspace{0.3cm}


\begin{cmt*}{R3C2}{} 

The Z-order space-filling curve serialization is a key component of the algorithm, but its presentation is not clear enough. From Algorithm 1, it is still difficult to tell how we can take an arbitrary sequence of points in any permutation and convert them into a sequence. There is also no explanation or citation on why they key property in Eq. (9) will be achieved by this approach. Please add more descriptions for the algorithm and explain how it guarantees this key property.

Additionally, is the Z-order space-filling curve serialization invariant to permutation of point enumeration and global rotations? (i.e., if we permute the points in the input sequence, does it lead to the same output sequence? If we globally rotate the input point sequence, does it lead to the same output sequence up to the same rotation?) If these properties are not met, then permuting or rotating the input sequence could potentially lead to different registration results, so I believe it is worth having some discussions here. 

\end{cmt*}
\vspace{0.1cm}
\noindent
\underline{\textbf{Response:}}
\vspace{0.2cm}

We clarify that our Z-order serialization is strictly invariant to point permutation but sensitive to global rotation. Since the Z-order sequence is generated by sorting points based on their spatial coordinates (Morton codes), the resulting sequence is deterministic and completely independent of the input enumeration order. \textbf{Our additional experiments confirm this}: randomly shuffling the input points (w random) yields results nearly identical to the baseline (RRE 0.160$^\circ$ vs. 0.161$^\circ$), proving that our method is robust to unstructured point storage. Regarding rotation, we acknowledge that the grid-based nature of Z-order makes it coordinate-dependent. As shown in our stress tests, applying large global rotations (30$^\circ$-90$^\circ$) without retraining leads to performance degradation (RR drops from 100\% to 83.6\%-45.7\%). This confirms that Z-order does not naturally possess rotational invariance like point-wise networks. However, this is a conscious design trade-off to achieve linear-complexity spatial modeling; in practical applications (e.g., autonomous driving) where gravity is aligned or training data covers the orientation distribution, our method achieves state-of-the-art precision (RRE 0.161$^\circ$) significantly surpassing rotation-invariant baselines.

\vspace{0.3cm}

\begin{table}[t]
\centering
\small
\caption{Stress test under input shuffling and large global rotations (without retraining).}
\label{tab:zorder_stress}
\begin{tabular}{l|ccc}
\toprule
Setting & RTE (cm) & RRE ($^\circ$) & RR (\%) \\
\midrule
MT-PCR & 2.55 & 0.161 & 100.0 \\
Random shuffle & 2.58 & 0.160 & 100.0 \\
Rotation 30$^\circ$ & 1.47 & 1.185 & 83.6 \\
Rotation 60$^\circ$ & 3.38 & 1.48 & 51.3 \\
Rotation 90$^\circ$ & 4.01 & 1.67 & 45.7 \\
\bottomrule
\end{tabular}
\end{table}
